Neoplatonic solids

A \emph{6-net} is a simplicial triangulation of the $2$-sphere with maximum degree $\leq 6$. Experiments suggest that every $6$-net admits a unique realization as an undented Euclidean polyhedron built from unit equilateral triangles, and a unique realization as an ideal equilateral hyperbolic polyhedron. We call these \emph{neoplatonic solids} and \emph{ideal neoplatonics}. A net is \emph{prime} if every 3-cycle bounds a face. A computer-assisted proof shows that every prime $6$-net with $v \leq 50$ has a unique realization as a convex ideal neoplatonic. Numerical homotopy from this realization yields an approximate Euclidean neoplatonic, and a computer-assisted proof shows that a true Euclidean neoplatonic lies nearby, though we do not prove uniqueness. Using the separating-triangle decomposition, we extend Euclidean existence to all $10{,}412{,}340$ $6$-nets with $v\leq50$, counted up to combinatorial isomorphism.

==> euclidean_gallery.tex <==
% Euclidean neoplatonic gallery -- generated by make_euclidean_gallery.py
% \input this file after the section heading in abcd.tex
% Requires: \usepackage{geometry} (already in abcd.tex)

\begin{figure}[h!]
\centerline{%
\includegraphics[width=123pt]{figures/e/CCAE.png}%%
\includegraphics[width=123pt]{figures/e/CCCACAAE.png}%%
\includegraphics[width=123pt]{figures/e/CCCACACAAE.png}%
}
\centerline{%
\includegraphics[width=185pt]{figures/e/CCCACACACAAE.png}%%
\includegraphics[width=185pt]{figures/e/CCCACACCAABE.png}%
}
\centerline{%
\includegraphics[width=123pt]{figures/e/CCCACACACACAAE.png}%%
\includegraphics[width=123pt]{figures/e/CCCACACACCAABE.png}%%
\includegraphics[width=123pt]{figures/e/CCCACCACACAAAE.png}%
}
\caption{The smallest Euclidean neoplatonics ($v=4,6,7,8,8,9,9,9$).}
\label{e_small}
\end{figure}


\begin{figure}[htbp]
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACCAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACCACADEE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACCACACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACCACACACAAAE.png}%
}
\caption{$v=10$.}
\label{e10}
\end{figure}


\clearpage
\newgeometry{top=0.6in,bottom=0.8in}
\clearpage
\begin{figure}[htbp]
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACCAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACACCACACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCACACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCACACACAABE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACACCACCACADAEE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACCACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACCACACACACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/3\relax]{figures/e/CCCACCACACCACAADEE.png}%
}
\caption{$v=11$.}
\label{e11}
\end{figure}

\clearpage
\begin{figure}[htbp]
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACACACACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACACCAACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACACCACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACACCACACACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACACCACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCAACACACCAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACACAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACACACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACACACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACCACACAAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACCACACAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACACCACCACACAABAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACCACAACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACCACACAAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACCACACAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACCACACDEAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACACCACACDEABE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACCACACAACADEE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCACCACCACACACAAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/4\relax]{figures/e/CCCCACCACACACAACAAAE.png}%
}
\caption{$v=12$.}
\label{e12}
\end{figure}

\begin{comment}
\clearpage
\begin{figure}[htbp]
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACACACACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACCAACACACCAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACCACACAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACCACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACCACACACACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACACCACACACACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACACACAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACACACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACACACACCAAABE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACCACACAAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACCACACAACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACCACACAACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACCACACAACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACACCACCACACACAAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACAACCACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACACACACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACACACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACACACCAACADEE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACAACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACAACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACAACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACACAAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACACAAABE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACACAABBE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACCAABAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACACCACACCAABABE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACCACACAACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACCACACACAACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACCACCACAACADEBE.png}%%
\includegraphics[width=\dimexpr\textwidth/5\relax]{figures/e/CCCACCACCACCACACAADEBE.png}%
}
\caption{$v=13$.}
\label{e13}
\end{figure}

\clearpage
\begin{figure}[htbp]
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACACACACACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCAACACACCAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACAACACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACAACCAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACACAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACACACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACACCACACACACCAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCAACACACCAACACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACAACCACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACAACCACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACAACACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACACACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACACACACCAACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACAACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACAACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACAACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACAACACDEAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACACAAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACACAABCAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACACAACAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACACACAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACACCACCACACACACAABAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACAACCACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACACACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACACACACAABE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACCAACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACCAACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACCACACADEAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACACACCACACADEBE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACAACACAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACAACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACAACACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACAAACAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACAABCAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACAACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACAACDEAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACACAAAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACACAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACACACAADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACCAACAAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACACCACACCAACAADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACAACACCAABAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACAACAACAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACAACACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACAACCAAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACACAACAAAE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACACAACAABE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACACACACAACADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACCACAACACDEAAE.png}%
}
\centerline{%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACCACACAACAADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACCACACAACDEDEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCACCACCACACACAAADEE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCACCCACCACCACAACDEDEBE.png}%%
\includegraphics[width=\dimexpr\textwidth/6\relax, totalheight=\dimexpr3\textwidth/20\relax, keepaspectratio=false]{figures/e/CCCCACCACACACACACAACAAAE.png}%
}
\caption{$v=14$.}
\label{e14}
\end{figure}
\end{comment}

\clearpage
\restoregeometry


==> gemdef.tex <==
\usepackage{wasysym}

\def\wasyfamilybold{\fontencoding{U}\fontfamily{wasy}\fontseries{b}\selectfont}

\newsavebox{\gembox}

\newcommand{\gem}{%
  {\mathord{%
    \mathchoice%
      {\gemresize{\displaystyle}}%
      {\gemresize{\textstyle}}%
      {\gemresize{\scriptstyle}}%
      {\gemresize{\scriptscriptstyle}}%
  }}%
}

\newcommand{\gemresize}[1]{%
  \sbox{\gembox}{$#1A$}%
  \resizebox{\wd\gembox}{\ht\gembox}{\wasyfamilybold\gemini}%
}

